SelfReg-UNet: Self-Regularized UNet for Medical Image Segmentation

Since its introduction, UNet has been leading a variety of medical image segmentation tasks. Although numerous follow-up studies have also been dedicated to improving the performance of standard UNet, few have conducted in-depth analyses of the underlying interest pattern of UNet in medical image segmentation. In this paper, we explore the patterns learned in a UNet and observe two important factors that potentially affect its performance: (i) irrelative feature learned caused by asymmetric supervision; (ii) feature redundancy in the feature map. To this end, we propose to balance the supervision between encoder and decoder and reduce the redundant information in the UNet. Specifically, we use the feature map that contains the most semantic information (i.e., the last layer of the decoder) to provide additional supervision to other blocks to provide additional supervision and reduce feature redundancy by leveraging feature distillation. The proposed method can be easily integrated into existing UNet architecture in a plug-and-play fashion with negligible computational cost. The experimental results suggest that the proposed method consistently improves the performance of standard UNets on four medical image segmentation datasets. The code is available at \url{https://github.com/ChongQingNoSubway/SelfReg-UNet}

==> cut_table.tex <==
% \begin{table}[]
% \centering
% \caption{}
% \label{tab:my-table}
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{l|c|c|c|c} 

% \hline
% \textbf{Methods} & \textbf{Avg DSC} & \textbf{RV} & \textbf{Myo} & \textbf{LV} \\
% \hline
% % R50 + UNet & 87.55 & 87.10 & 80.63 & 94.92 \\
% R50 + AttnUNet & 86.75 & 87.58 & 79.2 & 93.47 \\
% ViT + CUP & 81.45 & 81.46 & 70.71 & 92.18 \\
% % R50 + VIT + CUP & 87.57 & 86.07 & 81.88 & 94.75 \\
% UNet & 89.68 & 87.17 & 87.21 & 94.68 \\
% TransUNet & 89.71 & 86.67 & 87.27 & 95.18 \\
% SwinUNet  & 88.07 & 85.77 & 84.42 & 94.03 \\
% LeVit-Unet & 88.21 & 85.56 & 84.75 & 94.32\\
% Hiformer & 90.82 & 88.55 & 88.44 & 95.47\\
% PVT - CASCADE  & 90.45 & 87.20 & 88.96 & 95.19 \\
% \hline
% \rowcolor{blue!8}
% Our + Unet  & \underline{91.43} & 88.92 & 89.49 & 95.88\\
% \rowcolor{blue!8}
% $\Delta$  & \textcolor{red}{$+1.75$} & \textcolor{red}{$+1.75$} & \textcolor{red}{$+2.28$}& \textcolor{red}{$+1.20$}\\ 
% \hline
% \rowcolor{blue!8}
%  Our + SwinUNet & \textbf{91.49} & 89.49 & 89.27 & 95.70 \\ 
% \rowcolor{blue!8}
% $\Delta$  & \textcolor{red}{$+3.42$} & \textcolor{red}{$+3.72$} & \textcolor{red}{$+4.85$}& \textcolor{red}{$+1.67$}\\ 
% \hline
% \end{tabular}%
% }
% \end{table}



% \begin{table}[]
% \centering
% \caption{}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc}
% \hline
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{Glas}} & \multicolumn{2}{c}{\textbf{MoNuSeg}} \\
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{ \textbf{DSC (\%)}} &\multicolumn{1}{c}{ \textbf{IOU (\%)}}& \multicolumn{1}{c}{ \textbf{DSC (\%)}} &\multicolumn{1}{c}{\textbf{ IOU (\%)}}  \\
% \hline
% U-Net  & 85.45$\pm$1.25 & 74.78$\pm$1.67 & 76.45$\pm$2.62 & 62.86$\pm$3.00 \\
% UNet++  & 87.56$\pm$1.17 & 79.13$\pm$1.70 & 77.01$\pm$2.10 & 63.04$\pm$2.54 \\
% AttUNet & 88.80$\pm$1.07 & 80.69$\pm$1.66 & 76.67$\pm$1.06 & 63.47$\pm$1.16 \\
% MRUNet & 88.73$\pm$1.17 & 80.89$\pm$1.67 & 78.22$\pm$2.47 & 64.83$\pm$2.87 \\
% TransUNet & 88.40$\pm$0.74 & 80.40$\pm$1.04 & 78.53$\pm$1.06 & 65.05$\pm$1.28 \\
% MedT & 85.92$\pm$2.93 & 75.47$\pm$3.46 & 77.46$\pm$2.38 & 63.37$\pm$3.11 \\
% SwimUnet & 89.58$\pm$0.57 & 82.06$\pm$0.73 & 77.69$\pm$0.94 & 63.77$\pm$1.15 \\
% UCTransNet  & 90.18$\pm$0.71  & 82.96$\pm$1.06  & 79.08$\pm$0.67 & 65.50$\pm$0.91 \\
% \hline
% \rowcolor{blue!8}
% Our + Unet & \underline{90.93$\pm$0.20}  & \underline{84.08$\pm$0.41}  & \textbf{80.18$\pm$0.19} & \textbf{67.07$\pm$0.29} \\
% \rowcolor{blue!8}
% $\Delta$  & \textcolor{red}{$+5.48$} & \textcolor{red}{$+9.3$} & \textcolor{red}{$+3.73$}& \textcolor{red}{$+4.21$}\\ 
% \hline
% \rowcolor{blue!8}
% Our + SwinUnet & \textbf{91.62$\pm$0.16}  & \textbf{85.29$\pm$0.30}  & \underline{79.38$\pm$0.15} & \underline{65.87$\pm$0.21} \\
% \rowcolor{blue!8}
% $\Delta$  & \textcolor{red}{$+2.04$} & \textcolor{red}{$+3.23$} & \textcolor{red}{$+1.69$}& \textcolor{red}{$+2.10$}\\

% \hline

% \end{tabular}
% }
% \end{table}

==> results_cut.tex <==
The results in Synapse dataset are presented in Table~\ref{tab:synapse}. 
The main observation is our proposed losses substantially enhance average DSC by 3.84\% and 1.41\% for original Unet and swinUnet, respectively. Consequently, our methods outperform the SOTA HiFormer in the Synapse dataset, exhibiting improvements of 0.05\% and 0.25\% in average DSC, respectively. Compared with Hiformer, TransUnet, Unet, and swinUnet~\cite{unet,swimunet,hiformer,transUnet}, the performance gains primarily derive from tackling challenging organ segmentation tasks such as the gallbladder, left kidney, right kidney and pancreas, as illustrated in Fig~\ref{fig:seg1} and Table~\ref{tab:synapse}. These findings indicate that the proposed loss function effectively provides semantic supervision, preserving fine and detailed shape information.

Regarding the ACDC dataset results shown in Table~\ref{tab:addc}, we observe consistent improvements (avg DSC) of 1.75\% and 3.42\% based on the original Unet and SwinUnet architectures. Compared with SOTA HiFormer~\cite{hiformer}, our Unet and swinUnet methods demonstrate enhancements of 0.6\% and 0.67\% in average DSC, respectively. The superior performance underscores generalization and robustness capabilities.

A similar enhancement by our proposed loss can also be observed in Glas and MoNuSeg datasets. As shown in Table~\ref{tab:glas}, compared to the original SwinUnet, we observed DSC improvements of 2.04\% and 1.69\% and IOU improvements of 3.23\% and 2.10\% for Glas and MoNuSeg, respectively. 
Compared to the original Unet, we achieved DSC improvements of 5.48\% and 3.73\%, and IOU enhancements of 9.3\% and 4.21\% for Glas and MoNuSeg, respectively. As a result, our methods exhibit superior performance over the previous state-of-the-art method, UCTransNet, with 0.7\% and 1.1\% DSC gain in both datasets, respectively. Fig~\ref{fig:seg2} demonstrates that our method notably improves performance for both original ones. Notably, Unet with optimized skip connections (e.g., UCTTransNet~\cite{uctransunet}) leads to irrelevant segmentation and incomplete shapes. Especially segments resembling the background (last row). We conjecture that these methods fail to address semantic loss. While SwinUnet, with our proposed loss, demonstrates results that are closely comparable to the ground truth, featuring full shapes and clear backgrounds, particularly in the second sample (the last one of the second row in Fig~\ref{fig:seg2}). These observations support that our approach can provide contextual supervision, ensuring correct semantics across blocks and preventing the learning of irrelevant features.
